Linking Anomalous Behaviour with Stellar Properties: An Unsupervised Exploration of TESS Light Curves

With the upcoming plethora of astronomical time-domain datasets and surveys, anomaly detection as a way to discover new types of variable stars and transients has inspired a new wave of research. Yet, the fundamental definition of what constitutes an anomaly and how this depends on the overall properties of the population of light curves studied remains a discussed issue. Building on a previous study focused on Kepler light curves, we present an analysis that uses the Unsupervised Random Forest to search for anomalies in TESS light curves. We provide a catalogue of anomalous light curves, classify them according to their variability characteristics and associate their anomalous nature to any particular evolutionary stage or astrophysical configuration. For anomalies belonging to known classes (e.g. eclipsing binaries), we have investigated which physical parameters drive the anomaly score. We find a combination of unclassified anomalies and objects of a known class with outlying physical configurations, such as rapid pulsators, deep eclipsing binaries of long periods, and irregular light curves due to obscuration in YSOs. Remarkably, we find that the set of anomalous types differ between the Kepler and TESS datasets, indicating that the overall properties of the parent population are an important driver of anomalous behaviour.

==> Tables/final_results_w_notes_head.tex <==
\begin{longtable}{cccccccccccc}
\toprule
        tic\_id &                   designation &          ra &        dec &  main\_type &                             other\_types &  weirdness & sectors & weirdness>0.9 & weirdness>0.6 & weirdness<0.6 &        Notes \\
\midrule
\endhead
\midrule
\multicolumn{12}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
 TIC 471013946 &  Gaia DR2 2513021854931769344 &   33.821292 &   0.244569 &        WD* &                     *  |WD*|WD*|WD*|WD* &   0.989290 &     [4] &           [4] &            [] &            [] &            0 \\
 TIC 166463090 &  Gaia DR2 6670392146960681984 &  298.835020 & -48.282248 &   gammaDor &                         *  |UV |IR |gD* &   0.989262 &    [13] &          [13] &            [] &            [] &            0 \\
 TIC 177932603 &  Gaia DR2 3052092481686246016 &  107.658294 &  -7.122892 &   deltaCep &                          V* |cC*|*  |IR &   0.987706 &     [7] &           [7] &            [] &            [] &            0 \\
 TIC 444535842 &   Gaia DR2 510991333155346688 &   19.837507 &  62.301401 &        NaN &                                     NaN &   0.987691 &    [24] &          [24] &            [] &            [] &  [artefact ] \\
  TIC 30317282 &  Gaia DR2 4661514377893838464 &   74.272331 & -68.414734 &        EB* &                          *iA|EB*|*  |IR &   0.987162 &     [7] &           [7] &            [] &            [] &            0 \\
 TIC 439869954 &  Gaia DR2 2497895053130247040 &   43.384666 &  -0.562453 &        WD* &  WD*|blu|UV |*  |G  |*  |PM*|IR |WD*|** &   0.987156 &     [4] &           [4] &            [] &            [] &            0 \\
 TIC 142867174 &  Gaia DR2 5054768627234519552 &   50.837600 & -32.270100 &        NaN &                                     NaN &   0.986632 &     [4] &           [4] &            [] &            [] &            0 \\
 TIC 178366477 &  Gaia DR2 3071240270519385856 &  123.327106 &  -1.057903 &  CataclyV* &                                 ev |CV* &   0.986457 &     [7] &           [7] &            [] &            [] &            0 \\
 TIC 149894385 &  Gaia DR2 5587836255503080576 &  116.769000 & -34.372400 &        NaN &                                     NaN &   0.986149 &     [8] &           [8] &            [] &            [] &            0 \\
 TIC 444000734 &                           NaN &  131.365000 &  10.914900 &        PM* &                         *  |IR |*  |PM* &   0.986069 &     [7] &           [7] &            [] &            [] &            0 \\
\end{longtable}


==> Tables/summary.tex <==
\begin{table}[h]
    \begin{tabular}{cccccc}
    \toprule
        tic\_id & Weirdness & Reference & Notes
        (1) & (2) & (3) & (4) \\
    \midrule
 TIC 21505340  & 0.96 & \cite{Littlefield2021} & Quasi-periodic oscillations in WD star\\
 TIC 157376469 & 0.96 & \cite{Pan2021} (Binary system of K-type main sequence stars)\\
 TIC 63328020  & 0.95 & \cite{Rappaport2021} (dipole pulsation mode in the eclipsing binary)\\
 TIC 264509538 & 0.50 & \cite{Shi2020} (Pulsations of the Rapidly Oscillating Ap Star)\\
 TIC 229804573 & 0.95 & \cite{Borkovits2021}(compact hierarchical quadruple system)\\
 TIC 234523599 & 0.96 & \cite{Bakos2018} (A giant planet transiting an M3 dwarf star - clear transit events)\\
 TIC 257459955 & 0.91 & \cite{Bell2019} (WD - evolved compact pulsators)\\
 TIC 278659026 & 0.73 & \cite{Charpinet2019} (g-mode hot B subdwarf pulsator)\\
 TIC 38586082  & 0.86 & \cite{Khalack2019} (Chemically peculiar variable star of alpha2 CVn type)\\
    \bottomrule
    \end{tabular}
    \label{tab:data_table}
\end{table}

% - TIC 21505340 (TX col) - weirdness = 0.96 - \cite{Littlefield2021} (Quasi-periodic oscillations in WD star)\\
% - TIC 157376469 (TYC 7037-89-1) - weirdness = 0.96 - \cite{Pan2021} (Binary system of K-type main sequence stars)\\
% - TIC 63328020 (NSVS 5856840) - weirdness = 0.95 - \cite{Rappaport2021} (dipole pulsation mode in the eclipsing binary)\\
% - TIC 264509538 (KOI-7362) - weirdness = 0.50 - \cite{Shi2020} (Pulsations of the Rapidly Oscillating Ap Star)\\
% - TIC 229804573 (BG Ind) - weirdness = 0.95 - \cite{Borkovits2021}(compact hierarchical quadruple system)\\
% - TIC 234523599 (HATS-71b) - weirdness = 0.96 - \cite{Bakos2018} (A giant planet transiting an M3 dwarf star - clear transit events)\\
% - TIC 257459955 (G 272-B2A) - weirdness = 0.91 - \cite{Bell2019} (WD - evolved compact pulsators)\\
% - TIC 278659026 (EC 21494-7018)- weirdness = 0.73 - \cite{Charpinet2019} (g-mode hot B subdwarf pulsator)\\
% - TIC 38586082 (HD 27463) - weirdness = 0.86 - \cite{Khalack2019} (Chemically peculiar variable star of alpha2 CVn type)\\
